Graph minimization, focusing on the example of 5-chromatic unit-distance graphs in the plane

We introduce a new graph minimization method, in which it is required to preserve some graph property and there is an effective procedure for checking this property. We applied this method to minimize 5-chromatic unit-distance graphs and obtained a graph with 509 vertices and 2442 edges.

==> table1.tex <==
%-------------------------------------------------
\begin{table}[!b]
{
\caption{Main results}
\label{tres}
\smallskip

{
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multicolumn{2}{c|}{graph type} &\!sym\!	&$A$ &$M$ &edges	&set	\\
\hline
\hline
M-type graph	&M6A	&1	&	&509	&2442			\\
	&	&1	&	&510	&2502			\\
\hline
$L$-subgraph &M6A	&1	&412	&374	&1860-1884	&1092	\\
	&	&2	&402	&374	&1868-1884	&78	\\
	&	&1\,(2)	&457	&375	&1920-1930	&282	\\
	&	&3\,(6)	&451	&376	&1890-1947	&96	\\
\cline{2-7}
	&M6B	&2	&402	&374	&1864-1880	&78	\\
	&	&1\,(2)	&403	&375	&1916-1926	&66	\\
\cline{2-7}
	&M6C	&2	&382	&374	&1872		&76	\\
\hline
$S$-subgraph &M6A &1	&166	&136	&564-567	&8	\\
\cline{2-7}
	&M6B	&1	&172	&141	&594-595	&4	\\
\cline{2-7}
	&M6C	&1	&167	&150	&639-651	&28	\\
\hline
mono-pair   &$8/3$	    &1\,(4)	&391	&367	&1822		&27	\\
\cline{2-7}
            &$8/\sqrt3$	&4	    &433	&421	&2094-2106	&7	\\
\hline
non-mono-pair 	&$3$    &4      &226	&214	&977    	&2	\\
\cline{2-7}
             	&$7/3$  &4      &343	&319	&1524-1536	&34	\\
\cline{2-7}
             	&$5/3$  &1      &335	&315	&1497-1504	&17	\\
\cline{2-7}
             	&$1/3$  &4      &312	&312	&1502   	&1	\\
\cline{2-7}
	   &$\sqrt{11/3}$	&2      &309	&309	&1528		&1	\\
\hline
non-mono-triple &$\sqrt7$  &1  &180	 &157	&626-638	&51	\\
\cline{2-7}
                &$\sqrt5$  &1  &265	 &265	&1293   	&1	\\
\cline{2-7}
                &$\sqrt3$  &1  &238	 &221	&1006-1013	&120 \\
\cline{2-7}
            &$\sqrt{5/3}$  &3  &250	 &250	&1116   	&1	\\
\cline{2-7}
            &$\sqrt{1/3}$  &1  &292	 &265	&1246-1258	&1020	\\
\hline
\end{tabular}

}
}
\end{table}



==> table2.tex <==
%-------------------------------------------------
%\newpage

\begin{table}[!t]
{
\caption{Orbit comparison of some $L$-subgraphs. 
The following orbits are filled in the same way in all considered graphs and are not shown here (see~table \ref{tl}, where they are marked in gray in the "orbits" column):
\small
$(0,0,0,0)$, $(0,0,4,0)$, $(12,0,0,0)$, $(0,0,8,0)$, $(6,2,0,0)$, $(2,0,0,2)$, $(6,0,0,2)$, $(10,0,0,2)$, $(0,2,2,0)$, $(4,0,0,4)$, $(14,0,0,2)$, $(0,2,6,0)$, $(6,0,10,0)$, $(6,0,0,6)$, $(0,4,4,0)$, $(2,0,4,2)$, $(4,0,2,2)$, $(2,0,8,2)$, $(8,0,2,2)$, $(10,0,4,2)$, $(14,0,2,4)$.
}
\label{tcmp}
\smallskip

{
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
            & \multicolumn{4}{c|}{$M$}  & \multicolumn{4}{c}{$\{M\}$}  \\
\cline{2-9}
orbit      &374 &375 &382 &393 & 376   & 375  & 374  & 374  \\
\cline{2-9}
 & \multicolumn{2}{c|}{M6A\&B}  & \multicolumn{2}{c|}{M6A}  & 
 M6A  & \multicolumn{2}{c|}{M6A\&B}  & M6C  \\
\hline
\hline
 (4,0,0,0)  & 6  & 4  & 6  & 6  & 3     & 4    & 6    & 6    \\
 (0,0,0,4)  & 3  & 0  & 0  & 0  & 0     & 0    & 3    & 3    \\
 (0,0,12,0) & 6  & 6  & 0  & 0  & 6     & 6    & 6    & 6    \\
\hline
 (0,0,2,2)  & 8  & 6  & 0  & 0  & 6     & 6    & 6-8  & 8    \\
 (0,0,6,6)  & 6  & 0  & 0  & 0  & 0-3   & 0    & 6    & 6    \\
 (8,0,0,4)  & 0  & 0  & 6  & 6  & 0     & 0    & 0    & 0    \\
 (0,0,2,6)  & 6  & 6  & 6  & 6  & 6     & 6    & 6    & 6    \\
\hline
 (12,2,2,0) & 12 & 12 & 12 & 15 & 12    & 12   & 12   & 12   \\
 (2,0,6,4)  & 2  & 4  & 6  & 0  & 0-12  & 0-4  & 0-8  & 0-8  \\
 (4,0,6,2)  & 12 & 12 & 12 & 15 & 12    & 12   & 12   & 12   \\
 (4,0,4,4)  & 0  & 0  & 3  & 6  & 0-3   & 0    & 0    & 0    \\
 (8,0,6,2)  & 12 & 12 & 12 & 6  & 12    & 12   & 12   & 12   \\
 (6,2,4,0)  & 12 & 24 & 24 & 21 & 18-24 & 24   & 12   & 12   \\
 (2,0,2,4)  & 8  & 10 & 9  & 17 & 9-12  & 10   & 8-10 & 8    \\
 (8,0,4,4)  & 12 & 12 & 12 & 12 & 0-12  & 12   & 12   & 12   \\
 (12,2,6,0) & 0  & 0  & 0  & 6  & 0-12  & 0    & 0    & 0    \\
 (4,0,10,2) & 0  & 6  & 0  & 0  & 0-12  & 2-6  & 0-4  & 0    \\
 (10,0,2,4) & 10 & 8  & 0  & 0  & 0-12  & 8-12 & 4-12 & 4-12 \\
 (6,0,4,6)  & 0  & 0  & 3  & 6  & 0     & 0    & 0    & 0    \\
 (6,2,8,0)  & 12 & 6  & 24 & 24 & 0-12  & 6-10 & 8-12 & 12   \\
\hline
\end{tabular}

}
}
\end{table}


